Near-Field Measurement System for the Upper Mid-Band

The upper mid-band (or FR3, spanning 6-24 GHz) is a crucial frequency range for next-generation mobile networks, offering a favorable balance between coverage and spectrum efficiency. From another perspective, the systems operating in the near-field in both indoor environment and outdoor environments can support line-of-sight multiple input multiple output (MIMO) communications and be beneficial from the FR3 bands. In this paper, a novel method is proposed to measure the near-field parameters leveraging a recently developed reflection model where the near-field paths can be described by their image points. We show that these image points can be accurately estimated via triangulation from multiple measurements with a small number of antennas in each measurement, thus affording a low-cost procedure for near-field multi-path parameter extraction. A preliminary experimental apparatus is presented comprising 2 transmit and 2 receive antennas mounted on a linear track to measure the 2x2 MIMO channel at various displacements. The system uses a recently-developed wideband radio frequency (RF) transceiver board with fast frequency switching, an FPGA for fast baseband processing, and a new parameter extraction method to recover paths and spherical characteristics from the multiple 2x2 measurements.

==> other/abstract_v0.tex <==
%
%However, existing wideband platforms for investigating FR3 potential are often costly or tailored to specific scenarios. Additionally, increasing antenna aperture sizes result in enlarged near-field regions, challenging conventional far-field modeling for evaluating users in these areas.
%To address these challenges, we have developed a novel experimental platform for a line-of-sight (LOS) multiple input multiple output (MIMO) system operating in the near field of the upper mid-band. Our platform includes a highly configurable FR3 up and down converter (Pi-Radio transceiver) board, enabling scalability to multiple user terminals and diverse antenna configurations. We aim to present a comprehensive demonstration of the system in the final manuscript.
%
%As an important frequency range for upcoming generations of mobile networks, the upper mid-band (or FR3, between 6-24 GHz) can provide a good balance between coverage and spectrum efficiency. To fully investigate its potential, wideband platforms are desired to implement and verify the system. However, existing FR3 platforms are either too costly or designed for specific scenarios. Moreover,  increased antenna aperture size makes the near-field region enlarge, and users located in the near-field cannot be well evaluated by conventional far-field modeling methods. In this work, we build a novel experimental platform for a line-of-sight (LOS) multiple input multiple out (MIMO) system operated in the near field of the upper-mid band. The platform consists of four components including a highly configurable FR3 up and down converter (Pi-Radio transceiver) board operating at FR3, and the platform is capable of scaling to multiple user terminals and different antenna configurations. We expect to demonstrate the entire system in the final manuscript. \textcolor{blue}{We are targeting on the technical area of ``B. MIMO Communications and Signal Processing"}.
%


==> other/conclusion_gan.tex <==
\section{Conclusion}
\label{sec:conclusion}
Wireless multi-path channels can exhibit complex statistical relationships 
across different frequencies which are difficult to capture via standard models such as \cite{3GPP38901}, particularly for mmWave and THz channels.
In this work, we have presented a general modeling methodology for deriving full double
directional models at multiple frequencies.  The methods use state-of-the-art neural networks
and make minimal a priori assumptions in the data.  As such, we show they are able to capture
interesting cross-frequency relations.  The current method is based on extensive ray tracing data. 
A natural extension, left as future work, will be to augment the data with real data as these become available.


==> other/raytracing.tex <==
\section{Urban Cellular Ray Tracing Data and Scattering Modeling}
\label{sec:raytracing}

\begin{figure}
  \centering
  \includegraphics[width=0.7 \linewidth]{figs/partial_beijing.jpg}
  \caption{Ray tracing simulation area representing a 550 $\times$ 380 $\text{m}^2$ region of Beijing, China.}
  \label{fig:beijing_map}
\end{figure}


Although our methodology is general,
we will demonstrate the methods on two frequencies:  $f_1=$\, \SI{28}{GHz}, 
as used in 5G systems today \cite{shafi20175g}, 
and $f_2=$\, \SI{140}{GHz}, a key sub-THz frequency targeted for 
potential 6G use cases \cite{giordani2020toward,rappaport2019wireless}.
While there have
been recent multi-frequency measurement
campaigns
\cite{huang2020multi,cui2020multi},
these measurements are 
enormously time-consuming and there are no current
datasets with sufficient data points for
training complex neural networks.
Thus, similar to several recent works \cite{XiaRanMez2020,Alkhateeb2019,khawaja2017uav}
we use a powerful ray tracing tool, Wireless InSite by Remcom \cite{Remcom} to generate data for training. 
\iftoggle{conference}{
Specifically, an area of Beijing, China, consisting of 550 $\times$ 380 square meters as shown in Fig.~\ref{fig:beijing_map}, is imported. Using similar parameters to 3GPP report \cite{3GPP38901}, we manually place 100 terrestrial receiving gNBs on the outside of buildings with \SI{10}{m} height, 
and transmitting UEs are placed at 320 locations on streets \SI{1.5}{m}. 
The deployment results in 100 $\times$ 320 $=$ 32000 links (i.e. gNB-UE pairs).
We run independent ray tracing simulations 
on these the two frequencies.
We set the maximum number of reflections as six and the maximum number of diffraction as one, and we limited the maximum number of paths of a link to 20.
In addition, the ray tracing tool only collects paths with a power of at least -250 dBm.
}
{
An area of Beijing, China, consisting of 1650 $\times$ 1440 square meters, has been imported. This representation of Beijing includes building and terrain data, as shown in Fig.~\ref{fig:beijing_map}.
To generate the data set, we manually placed 180 terrestrial receiving gNBs on the outside of the building with \SI{2}{m} height, imitating the typical locations of 5G PicoCell stations which are designed to serve the ground users. 
The transmitting UEs were placed at 120 locations on streets \SI{1.5}{m} high resembling street-level users.  These numbers are also consistent
with micro-cellular models in \cite{3GPP38901}.  

With the above gNBs and UEs configuration, there are total of 180 $\times$ 120 $=$ 21600 links (i.e. gNB-UE pairs). 
We ran independent ray tracing simulations 
on these links at
two frequencies:  $f_1=$\, \SI{2.3}{GHz}
and $f_2=$\, \SI{28}{GHz} -- typical values
for a sub-6 GHz and mmWave carrier
in commercial deployments today.

The materials will have different 
permittivity and conductivity values at different
frequency.  In this simulation, we use the values Table~\ref{table:material_para}. 
Furthermore, we set the maximum number of reflections as six and the maximum number of diffraction as one, and we limited the maximum number of paths of a link to 20. 

\begin{table}
\caption{Material Parameters$^{*}$}
\begin{center}
\begin{tabular}{c|c|c|c|c|}
\cline{2-5}
                                         & \multicolumn{2}{c|}{Earth Ground} & \multicolumn{2}{c|}{Buliding Wall} \\ \hline
\multicolumn{1}{|c|}{Frequency (GHz)}     & 2.3              & 28             & 2.3              & 28              \\ \hline
\multicolumn{1}{|c|}{Permittivity (F/m)} & 21.13            & 5.70           & 5.31             & 5.70            \\ \hline
\multicolumn{1}{|c|}{Conductivity (S/m)} & 0.47             & 9.50           & 0.07             & 9.50            \\ \hline
\multicolumn{4}{l}{$^{*}$Default value in Remcom database \cite{Remcom}}
\end{tabular}
\end{center} 
\label{table:material_para}
\end{table}
}

Critical to modeling the frequency dependence is the effect of diffuse
scattering, which is particularly prominent in the mmWave and THz
frequencies \cite{schecklman2011terahertz,ju2019scattering,xing2021millimeter}.
As part of our simulation, we enable the diffusing scattering model in the ray tracing tool which is based on the directive model developed by \cite{degli2007measurement}. A key parameter is the scattering
coefficient, $S$, which is the ratio of the scattered to incident
electric field.
Following measurements in  \cite{degli2007measurement}, 
we set the scattering coefficient 
 to $S=0.273$ for \SI{28}{GHz}, and $S=0.4$ for \SI{140}{GHz},
in which case, rays in \SI{140}{GHz} disperse more power on the forward lobe of diffuse scattered.
A diffuse scattering interaction is limited to the last interaction along a path before it reaches the receiver. This helps reduce the run time for diffuse scattering calculations. 


==> other/setup_v0.tex <==
\section{Proposed Measurement Platform}
In this paper, we present an experimental platform for near-field channel measurements in the upper mid-band. 
The system has four components:  
\begin{itemize}
    \item \textbf{Antenna:}  In the initial experiments two Vivaldi antennas will be mounted on a linear track.
    The Vivaldi antennas enable wideband operation across the full FR3 band and are readily manufacturable on standard
    PCBs.  The linear track has a motorized control to precisely adjust the separation with separation of up to \SI{2}{m}.

    \item \textbf{RF transceiver board}:
    The antennas will mate with an RF transceiver board manufactured by Pi-Radio that performs the up- and down-conversion to 2 TX and 2 RX IF streams. This two-stage up- and down-conversion is used to meet the out-of-band (OOB) and adjacent channel rejection ratio (ACLR) requirements and strict spectral masks. The transceiver board is built from commercial off-the-shelf (CoTS) parts. Importantly, the board
    enables fast frequency switching ($<1$\,\si{\micro\second}) to enable near simultaneous measurements across different frequencies.

    \item \textbf{Digital baseband system}:
    The FR3 front-end will be connected to a Xilinx RFSoC 4x2 \cite{xinlinx4by2}
    that will transmit and receive the sounding waveform.    
    We will use a sample rate of $f_s=1$\,\si{GHz} enabling high time resolution.
               
    \item \textbf{Host computer}: The host computer is used for non-real-time processing including loading the TX
    waveforms, capturing the RX waveforms, controlling the RF board and linear track, and performing offline processing.
\end{itemize}


The sounding waveform will consist of: (1) A preamble sent on both antennas for initial synchronization; followed by
(2) two reference signals sent from each TX antenna.  The reference signals will be repeatedly sent so that 
the channel will act as a circular convolution.  The receiver can then perform frequency domain correlation to extract the frequency-varying $2 \times 2$ MIMO channel.  The Pi-Radio board features a very accurate oven-controlled oscillator 
(OCXO) with error less than \SI{0.2}{ppb}~\cite{ocxo}.   
This accuracy enables very long integration periods.

The measurements will then be repeated at multiple displacements of the antennas through the linear track, thereby
collecting a number of $2 \times 2$ frequency-varying channel matrices.  These measurements may be non-coherent,
meaning there may be arbitrary phase rotations at the TX and RX at different TX and RX displacements.
Our next step is to synthesize the measurements to extract a near-field model.  We will follow a recent near-field model~\cite{hu2023parametrization} where each path is described by the location of a reflected transmitted point
and a rotation frame of reference.  
Finally, we will provide a method to extract these parameters from multiple non-coherent $2 \times 2$ measurements.




\begin{figure*}[ht]
\footnotesize
\centering
\includegraphics[width=0.99\linewidth]{figs/setup-1.pdf}
\caption{The architecture for the designed near-field FR3 platform with four components: two Vivaldi antennas on a linear track, a Pi-Radio two-channel FR3 transceiver board, a baseband system with RFSoC 4$\times$2, and a host computer.}
% \textcolor{red}{Change the diagram to replace the Keysight equipment and display 
% with a RFSoC 2x2.  Also replace the patch antennas with Vivaldi antennas. }
\label{fig:setup}
\end{figure*}

% \begin{figure*}[ht]
% \footnotesize
% \centering
% \includegraphics[width=0.8\linewidth]{fr3_chan_meas_4by4.pdf}
% \caption{The architecture for the designed platform.}
% \label{fig:system_extend}
% \end{figure*}





% \subsection{Overall Setup with $2\times2$ MIMO}
% As shown in Fig.~\ref{fig:system}, the proposed system has four components:


% \subsection{Scalability I: Operation with Multiple users}
% After verifying the functionality of the \gls{mimo} setup, the system will be extended to two receive terminals.  The terminals will be placed in a co-linear path from the transmitter at different distances in the near-field region.  Since the receive terminals have the same \gls{aod} from the transmitter, a standard \gls{mimo} system in the far-field would not be able to separate the receivers.   In this experiment, we will demonstrate that the designed system is capable of serving multiple users and separating them in the near-field.



% \subsection{Scalability II: $4\times4$ MIMO}
% To further demonstrate the potential of the designed platform, the two antennas on the linear track will be replaced by a fixed four-antenna system.  A rigid structure with multiple patch antennas will be fabricated.  Each patch antenna will have a feed from the reverse side of the structure via an \gls{sma} cable.  This way, the \gls{rf} system can be integrated into any subset of the antennas to experiment with different antenna placements.  The exact number and dimensions of the structure will be approximately  1m$\times$1m in dimension and approximately 16 or 64 antenna locations.

% As an example shown in Fig.~\ref{fig:system_extend}, the \gls{rf} transceiver functions for the four channels will be performed by two dual-channel Pi-Radio boards.  The Pi-Radio boards are designed to be frequency-locked.  Specifically, one board can supply the other board an \gls{lo}.  In this way, the four antennas can have a common \gls{lo}.  Since two boards are required for the transmitter and two for the receiver, this system requires four boards in total.

% On the transmit side, we will use an 8-channel RFSoC for the baseband in the test phase to measure the 4$\times$4 \gls{mimo} channel.  Once the channel is measured, we will move to the 4$\times$4 \gls{mimo} baseband system.

% \subsection{Expected results}
% We are expecting to demonstrate in the conference and the final manuscript that:
% \begin{itemize}
%     \item The proposed system could perform channel sounding at near fields with different numbers of users and antenna configurations.
%     \item The \gls{mimo} system operates as expected and shows performance enhancement compared to baseline systems.
% \end{itemize}


==> proof2d.tex <==
\section{Derivation of the distance formula for $d=2$}
\label{sec:proof_2d}

The distance is
\begin{align}
    d(\bsym{x}^r,\bsym{x}^t) = \| -\bsym{u}^r_0 + \bsym{x}^r-\bsym{x}^r_0 + s\bsym{R}(\phi) (\bsym{x}^t-\bsym{x}^t_0)\|,
\end{align}
where
\begin{equation}
    \phi = \phi^t + s\pi - \phi^r.  
\end{equation}
The directional derivative is:
\begin{align}
    \frac{\partial d(\bsym{x}^r, \bsym{x}^t)}{\partial \bsym{x}^r}
    &= \bsym{u}^r_0 -\bsym{x}^r + \bsym{x}^r_0 + s\bsym{R}(\phi) (\bsym{x}^t-\bsym{x}^t_0).
\end{align}


From \cite{hu2023parametrization}, we have that the distance
function is:
\begin{equation}
    d(\bsym{x}^r, \bsym{x}^t) = \|\bsym{d}_0 + \bsym{x}^r - \bsym{x}^r_0
        - \bsym{U}(\bsym{x}^t - \bsym{x}^t_0) \|
\end{equation}
where  $\bsym{d}_0$ is the vector from the RX reference
$\bsym{x}^r_0$ to the image point of the TX reference $\bsym{z}^t_0$,
\begin{equation}
    \bsym{d}_0 = \bsym{x}^r_0 - \bsym{z}^t_0.
\end{equation}
Let
\begin{align}
    c\tau &= \|\bsym{d}_0\|,\\
    \bsym{u}^r &= \bsym{d}_0, \\
    \bsym{u}^t &=  \bsym{U}\bsym{d}_0 \label{eq:urd}
\end{align}
So, to first order:
\begin{equation}
    d(\bsym{x}^r,\bsym{x}^t) = c\tau_0 - 
    (\bsym{u}^r)^\intercal (\bsym{x}^r - \bsym{x}^t)
    - (\bsym{u}^r)^\intercal (\bsym{x}^r - \bsym{x}^t)
\end{equation}
We know that 
\begin{align}
    \bsym{u}^r = \bsym{u}(\phi^r) = [\cos(\phi^r), \sin(\phi^r)] \\
    \bsym{u}^t = \bsym{u}(\phi^t) = [\cos(\phi^t), \sin(\phi^t)],
\end{align}
where $\phi^r$ and $\phi^t$ are the AoA and AoD.
Also, we know
\begin{equation}
    \bsym{u} = s \bsym{R}(\phi),
\end{equation}
for some $\phi$ and $s=\pm 1$.
From \eqref{eq:urd}, we have
\[
    \bsym{u}^r = \bsym{u}(\phi^r) = s R(\phi) \bsym{u}(\phi^t)
    = \bsym{u}(\phi^t + \phi + s\pi),
\]
Hence,

Then, the distance squared is:
\begin{align}
   \MoveEqLeft  d^2(\bsym{x}^r, \bsym{x}^t) 
   = (c\tau_0)^2  
    + \|\bsym{x}^r - \bsym{x}^r_0\|^2 +  \|\bsym{x}^r - \bsym{x}^r_0\|^2 \\
    & - c\tau_0 \bsym{u}(\phi^r)^\intercal(\bsym{x}^r - \bsym{x}^r_0)   - c\tau_0 \bsym{u}(\phi^t)^\intercal(\bsym{x}^t - \bsym{x}^t_0) 
\end{align}

Let $\bsym{R}(\phi)$ be the rotation matrix in $\mathbb{R}^2$:
\begin{equation}
    \bsym{R}(\phi):= \begin{bmatrix}
        \cos(\phi) & -\sin(\phi) \\
        \sin(\phi) &  \cos(\phi) 
    \end{bmatrix}.
\end{equation}
Write 
\begin{equation}
    \bsym{d}_0 = -c\tau[\cos(\phi^r), \sin \phi^r]^\intercal
    = -c\bsym{R}(\phi^r)\bsym{e}_x,
\end{equation}
where $c$ is the speed of light, $\tau$ is the time of flight
along the path, $\phi^r$ is the angle of arrival.
When $x^r = x^r_0$, $d$ simplifies to
\[
    d = \|-U^\intercal (x^r_0 - z_0^t) + x^t - x^t_0 \|
\]

Since $\bsym{U}$ is an orthogonal matrix in $p=2$ dimensions,
we can write:
\begin{equation}
    \bsym{U} = s \bsym{R}(\phi^t+\phi^r).
\end{equation}

